Revisiting the Membership, Multiplicity, and Age of the Beta Pictoris Moving Group in the Gaia Era

Determining the precise ages of young (tens to a few hundred Myr) kinematic (``moving") groups is important for placing star, protoplanetary disk, and planet observations on an evolutionary timeline. The nearby $\sim$25 Myr-old $\beta$ Pictoris Moving Group (BPMG) is an important benchmark for studying stars and planetary systems at the end of the primordial disk phase. Gaia DR3 astrometry and photometry, combined with ground-based observations and more sophisticated stellar models, permit a systematic re-evaluation of BPMG membership and age. We combined Gaia astrometry with previously published radial velocities to evaluate moving group membership in a Bayesian framework. To minimize the effect of unresolved stellar multiplicity on age estimates, we identified and excluded multi-star systems using Gaia astrometry, ground-based adaptive optics imaging, and multi-epoch radial velocities, as well as literature identifications. We estimated age using isochrone and lithium-depletion-boundary fitting with models that account for the effect of magnetic activity and spots on young, rapidly rotating stars. We find that age estimates are highly model-dependent; Dartmouth magnetic models with ages of 23$\pm$8 Myr and 33$^{+9}_{-11}$ Myr provide best fits to the lithium depletion boundary and Gaia $M_G$ vs. $B_{P}$-$R_{P}$ color-magnitude diagram, respectively, whereas a Dartmouth standard model with an age of 11$^{+4}_{-3}$ Myr provides a best fit to the 2MASS-Gaia $M_{K_S}$ vs. $B_{P}$-$R_{P}$ color-magnitude diagram.

==> extra.tex <==

%Isochrones are theoretical curves on a Hertszprung-Russell Diagram (HRD) or, the observational analog, a color-magnitude diagram, identifying a co-eval population of stars at different masses. In a HRD or CMD, the horizontal axis represents temperature (roughly mass or color, as a proxy) while the vertical axis is the star's intrinsic brightness (i.e., absolute magnitude or luminosity). For main sequence (MS) and pre-MS stars, the higher mass, hotter stars will generally reside toward the upper left of the diagram, while the cooler, lower mass stars will be toward the lower right. Stellar evolutionary tracks follow a single star's evolution over time in luminosity (magnitude) vs. effective temperature (color) space \citep{Kippenhahn2013}. This is illustrated in the right-side panel of  the dashed lines show the evolution of single stars (0.2, 0.5, 1.0, 1.3 M$_\odot$) from 1 Myr (green points) to 4 Gyr (magenta points) \citep{Somers2020}. Connecting contemporary points across the different evolutionary tracks produces an isochrone. Isochrone models from 10-50 Myr from the \citep{Baraffe2015} evolutionary models are plotted on a CMD in the left-side panel of  The CMD displays \textit{Gaia} absolute magnitude (denoted as M$_G$) vs. color (B$_{\rm P}$-R$_{\rm P}$). The absolute magnitude is computed from the apparent magnitude and distance (parallax). The color is the difference in apparent magnitudes in two passbands, B$_{\rm P}$ and R$_{\rm P}$, with the bluer magnitude preceding the redder by convention. From \textit{Gaia}, B$_{\rm P}$ stands for blue photometer and R$_{\rm P}$ stands for red photometer. Even within this small age range, it is clear how stars of different masses (B$_{\rm P}$-R$_{\rm P}$, by proxy) evolve differently over time, especially at the younger (10-30 Myr) ages, where greater offsets in the isochrones are visible at different ranges of B$_{\rm P}$-R$_{\rm P}$. Generally, younger isochrones are above and toward the right of older ones.% Once the MS is reached, it becomes much more difficult to discern differences in the isochrones, since a star's brightness and temperature are stable during its MS lifetime.

%For MS stars, the evolutionary models trace changes in luminosity and effective temperature due to surface gravity changes that result from nuclear fusion in stellar cores \citep{Angus2019}. Pre-MS evolution is distinct from MS evolution. For pre-MS stars, hydrogen burning has not yet begun; instead, the models trace the evolution of pre-MS stars fueled by gravitational contraction and deuterium fusion. Low-mass, pre-MS stars are fully convective, and the opacity in their interiors remains high until they reach temperatures hot enough to develop radiative cores and energy transfer becomes more efficient \citep{Kunitomo2017}. Before this occurs, their luminosity is largely a function of gravity (and radius), so they decrease in luminosity as they contract. This is illustrated by their vertical, downward evolution on the CMD (known as Hayashi tracks) in . This evolution occurs on the Kelvin-Helmholtz (KH) timescale, and varies by mass. Once a radiative core develops and opacity drops, stars will move to the left of the diagram due to temperature increase, as is shown in the 1.0 and 1.3 M$_\odot$ tracks in Fig.  The MS is reached when a star begins hydrogen burning and reaches thermal equilibrium, where a star will spend $\sim$80\% of its lifetime. The lowest mass stars (M dwarfs $\lessapprox2\;M_\odot$) are fully convective even on the main sequence, thus their pre-MS evolution on the CMD remains almost entirely vertical. 
 
%As mentioned, for pre-MS stars such as the BPMG members, there are large differences in the evolutionary phases of stars at different masses. The KH timescale for stars increases inversely with mass, with the highest mass ($> 8$ M$_\odot$) stars having KH radiative lifetimes shorter than their accretion time \citep{Hammerle2017}. Meanwhile, for the lower mass stars, the KH time is orders of magnitude longer than the accretion time \citep{Stahler1983}. In other words, massive stars evolve much more rapidly than low mass stars. Thus, very high mass stars may already be evolving off the MS at the same age, even at young ages \citep{Haemmerle2019}. Because of these contrasting behaviors, most evolutionary models do not span the very low to very high mass ranges.
 
 %A star’s position on a CMD or HRD is sensitive to several physical mechanisms such as surface activity, multiplicity, or reddening/extinction. There are many evolutionary model grids and isochrones in the literature, tailored for different phases of evolution, mass ranges, and more complex stellar activity \citep[e.g.,][]{Chabrier1997,Yi2001,Baraffe2015,Dotter2008,Dotter2016,Feiden2016,Haemmerle2019,Somers2020}, and each have their own systematics and caveats. Isochrone model fitting is the most widely used method for estimating stellar ages, and relies on precise photometric data and distance measurements (via parallax) to estimate an age for a stellar association, in addition to an appropriate choice of models. As evident in the right-hand panel of  there are significant effects of including magnetism and surface spots in the models, because they account for the elevated luminosity resulting from magnetic activity. While all of the isochrones indicate a 20 Myr age, the Dartmouth magnetic and SPOTS high spot fraction (f=0.85) models appear younger (above and to the right) of their more standard counterparts (Dartmouth standard, BHAC, SPOTS f=0.00). For the models to converge on the same locus, we would need to increase the ages of the magnetic and spot fraction models, thus, the magnetic and spot fraction models would assign older ages to the same sequence of stars. The models utilized in this study are further described in Sec. \ref{cmd}.
  
%LDB fitting is another age-dating method commonly applied to stellar associations, comparing surface Li abundances by temperature (again, color as a proxy; ). Measurements of surface Li abundances (equivalent width of the Li I 6708 Å line) in low-mass stars provide important information about their interior structures and nuclear ages \citep{Palla2007}. $^7$Li is depleted by proton reactions at a threshold of about 2.5 $\times 10^{6}$ K \citep{Burke_2004}. The LDB age estimate is the time it takes for internal temperatures to reach this threshold, and for lithium to be convected down into and destroyed these regions. We show the LDB curves from 10-30 Myr from the \citep{Baraffe2015} evolutionary models in Fig. to illustrate how the boundary changes with time; generally the Li gap widens with age. At younger ages, the LDB (the right-hand side of the trough) is at higher masses (smaller B$_{\rm P}$-R$_{\rm P}$), because it takes more time for the lower mass stars to reach the Li depletion temperature and for convective mixing to fully deplete Li. On the left-hand side of the boundary, photospheric temperatures are not high enough to destroy Li, and the onset of the radiative core structure leads to a halt in the Li depletion.
 
%The LDB appears in the mass range of stars near the hydrogen burning mass limit, which is a critical mass at which a star cannot sustain its surface luminosity through hydrogen burning ($\sim$0.1-0.3 M$_\odot$). These are low mass stars reaching internal temperatures hot enough to burn Li \citep{Baraffe2017}. This is a rapid process, as illustrated in Fig.  with the evolutionary tracks for 0.2, 0.5, 1.0, and 1.3 M$_\odot$ stars. For each track, there is a very steep drop-off in Li abundance, and for more the lowest mass tracks (0.2-0.5 M$_\odot$), lithium is fully depleted very quickly. Meanwhile some Li remains in the more Sun-like stars and the very low mass stars ($\lessapprox0.7$ M$_\odot$), which cannot reach the internal temperatures to burn lithium. The 20 Myr LDB from the various models used in this study (described in Sec. \ref{cmd}) are shown in  to illustrate how including magnetic and spot fraction effects change the LDB. Similar to the case of the isochrones, the 20 Myr Dartmouth magnetic and SPOTS f=0.00 models show younger LDBs (narrower) compared to the standard models. 
 
%For fully convective ($<$0.5 M${_\odot}$) M dwarf stars, lithium is fully destroyed within $\sim$50 Myr \citep{Bildsten_1997}. Mixing processes, such as overshooting, at the convective boundary have long posed a difficult obstacle in the evolutionary models \citep{Shaviv1973}, and the convective activity is further complicated by effects from rotation \citep{Baraffe2017}. However, LDB fitting provides a useful comparison to isochrone fitting and is resistant to some of the systematics and limitations of photometry-reliant age estimates. 

